CodeChain: Towards Modular Code Generation Through Chain of Self-revisions with Representative Sub-modules

Large Language Models (LLMs) have already become quite proficient at solving simpler programming tasks like those in HumanEval or MBPP benchmarks. However, solving more complex and competitive programming tasks is still quite challenging for these models - possibly due to their tendency to generate solutions as monolithic code blocks instead of decomposing them into logical sub-tasks and sub-modules. On the other hand, experienced programmers instinctively write modularized code with abstraction for solving complex tasks, often reusing previously developed modules. To address this gap, we propose CodeChain, a novel framework for inference that elicits modularized code generation through a chain of self-revisions, each being guided by some representative sub-modules generated in previous iterations. Concretely, CodeChain first instructs the LLM to generate modularized codes through chain-of-thought prompting. Then it applies a chain of self-revisions by iterating the two steps: 1) extracting and clustering the generated sub-modules and selecting the cluster representatives as the more generic and re-usable implementations, and 2) augmenting the original chain-of-thought prompt with these selected module-implementations and instructing the LLM to re-generate new modularized solutions. We find that by naturally encouraging the LLM to reuse the previously developed and verified sub-modules, CodeChain can significantly boost both modularity as well as correctness of the generated solutions, achieving relative pass@1 improvements of 35% on APPS and 76% on CodeContests. It is shown to be effective on both OpenAI LLMs as well as open-sourced LLMs like WizardCoder. We also conduct comprehensive ablation studies with different methods of prompting, number of clusters, model sizes, program qualities, etc., to provide useful insights that underpin CodeChain's success.

==> tables/apps_val_results_public_private_tests.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of APPS validation results by pass@1 (\%) on public vs. private test cases}
\begin{tabular}{ccccc}
\hline
Revision round & Introductory   & Interview      & Competition    & All            \\
\hline
\multicolumn{5}{c}{Public test cases}                                                   \\
\hline
Round 1        & 79.75          & 71.60          & 73.46          & 74.94          \\
Round 2        & 86.08          & 71.03          & 78.70          & 78.60          \\
Round 3        & 82.25          & 75.96          & \textbf{81.85} & 80.02          \\
Round 4        & \textbf{87.00} & \textbf{79.81} & 78.83          & \textbf{81.88} \\
Round 5        & 71.75          & 70.00          & 78.33          & 73.36          \\
\hline
\multicolumn{5}{c}{Private test cases}                                                   \\
\hline
Round 1        & 52.00          & 38.83          & 14.50          & 35.11          \\
Round 2        & 54.53          & 38.63          & 18.80          & 37.32          \\
Round 3        & 53.00          & 41.10          & \textbf{21.10} & \textbf{38.40} \\
Round 4        & \textbf{54.90} & \textbf{43.10} & 17.17          & \textbf{38.39} \\
Round 5        & 48.80          & 38.00          & 18.50          & 35.10        \\
\hline
\end{tabular}
\end{table}

==> tables/leetcode.tex <==
\begin{table}[htbp]
\centering
\small
\caption{Results on LeetCodeHardGym benchmark: results marked with $\dagger$ are reported from \citep{shinn2023reflexion} on a slightly different set of test samples.}
\begin{tabular}{lc}
\hline
Model          & pass@1         \\
\hline
GPT4           & 3.71           \\
CodeChain+GPT4 & \textbf{7.18}  \\
\hline
Codex $^\dagger$        & 3.60           \\
GPT4  $^\dagger$         & 7.50           \\
Reflexion+GPT4 $^\dagger$  & \textbf{15.00} \\
\hline
\end{tabular}
\end{table}
